SANPO: A Scene Understanding, Accessibility and Human Navigation Dataset

Vision is essential for human navigation. The World Health Organization (WHO) estimates that 43.3 million people were blind in 2020, and this number is projected to reach 61 million by 2050. Modern scene understanding models could empower these people by assisting them with navigation, obstacle avoidance and visual recognition capabilities. The research community needs high quality datasets for both training and evaluation to build these systems. While datasets for autonomous vehicles are abundant, there is a critical gap in datasets tailored for outdoor human navigation. This gap poses a major obstacle to the development of computer vision based Assistive Technologies. To overcome this obstacle, we present SANPO, a large-scale egocentric video dataset designed for dense prediction in outdoor human navigation environments. SANPO contains 701 stereo videos of 30+ seconds captured in diverse real-world outdoor environments across four geographic locations in the USA. Every frame has a high resolution depth map and 112K frames were annotated with temporally consistent dense video panoptic segmentation labels. The dataset also includes 1961 high-quality synthetic videos with pixel accurate depth and panoptic segmentation annotations to balance the noisy real world annotations with the high precision synthetic annotations. SANPO is already publicly available and is being used by mobile applications like Project Guideline to train mobile models that help low-vision users go running outdoors independently. To preserve anonymization during peer review, we will provide a link to our dataset upon acceptance. SANPO is available here: https://google-research-datasets.github.io/sanpo_dataset/

==> datasheet.tex <==
\title{SANPO Datasheet}
\maketitle

\section{Motivation}

\begin{enumerate}

\item \question{For what purpose was the dataset created? Was there a specific task in mind? Was there a
specific gap that needed to be filled? Please provide a description.}\\
\answer{SANPO was created to support research and development of computer vision based Assistive Technologies. Specifically, we are most interested in panoptic segmentation, depth-estimation, and related downstream challenges (obstacle avoidance, etc). Most existing datasets of this nature are either self-driving (not egocentric) or do not feature challenging outdoor scenarios.}

\item \question{Who created this dataset (e.g., which team, research group) and on behalf of which entity
(e.g., company, institution, organization)?}\\
\answer{The SANPO-Real dataset was created by researchers at Google LLC. SANPO-Synthetic was created by researchers at Parallel Domain with assistance from Google LLC.}

\item \question{Who funded the creation of the dataset? If there is an associated grant, please provide the
name of the grantor and the grant name and number.}\\
\answer{The SANPO dataset was funded by Google LLC.}

\item \question{Any other comments?}\\
\answer{We hope our dataset is useful to the community!}
\end{enumerate}

\section{Composition}

\begin{enumerate}
    \item \question{ What do the instances that comprise the dataset represent (e.g., documents, photos, peo-
ple, countries)? Are there multiple types of instances (e.g., movies, users, and ratings; people
and interactions between them; nodes and edges)? Please provide a description.}\\
\answer{Each instance in SANPO represents a session, comprising videos from one or two stereo cameras. We additionally provide the following annotations: depth maps for inferred from each stereo camera, and human-rated panoptic segmentations for the left video stream. We also provide session metadata (weather, time of day, etc), IMU positioning information, and other global metadata like camera intrinsics. SANPO-Synthetic includes similar data in the same format.}

\item \question{How many instances are there in total (of each type, if appropriate)?}\\
\answer{In total there are 2662 sessions.}

\item \question{Does the dataset contain all possible instances or is it a sample (not necessarily random)
of instances from a larger set? If the dataset is a sample, then what is the larger set? Is
the sample representative of the larger set (e.g., geographic coverage)? If so, please describe
how this representativeness was validated/verified. If it is not representative of the larger set,
please describe why not (e.g., to cover a more diverse range of instances, because instances
were withheld or unavailable).}\\
\answer{SANPO contains all usable sessions that were recorded.}

\item \question{Q8. What data does each instance consist of? “Raw” data (e.g., unprocessed text or images)
or features? In either case, please provide a description.}\\
\answer{Each instance in SANPO consists of RGB frames (as png files) and associated depth and segmentation annotation. Additionally, we also provide session level attributes and for each video camera pose trajectory is provided.}

\item \question{Is there a label or target associated with each instance? If so, please provide a description.}\\
\answer{We provide segmentation (png files) and depth annotations (floating-point arrays). Additionally, we provide session level attributes and for each video camera pose trajectory is provided.}

\item \question{Is any information missing from individual instances? If so, please provide a description,
explaining why this information is missing (e.g., because it was unavailable). This does not
include intentionally removed information, but might include, e.g., redacted text.
No and yes. No, because all the metadata fields for every instance are filled with valid values.}\\
\answer{Yes, for synthetic sessions we only provide one stereo camera and only one (left) video stream from it. Also we don't provide session level attributes for the synthetic data.}

\item \question{Are relationships between individual instances made explicit (e.g., users’ movie ratings,
social network links)? If so, please describe how these relationships are made explicit.}\\
\answer{Relationships between individual instances (e.g., sessions collected by the same volunteer or captured in nearby geographic locations) are not made explicit in our work.}

\item \question{Are there recommended data splits (e.g., training, development/validation, testing)? If
so, please provide a description of these splits, explaining the rationale behind them.}\\
\answer{We explicitly provide train and test session ids in corresponding text files to ensure reproducibility of results.}

\item \question{Are there any errors, sources of noise, or redundancies in the dataset? If so, please provide
a description.}\\
\answer{SANPO-Real may contain noisy segmentation or depth labels. Segmentation labels are combination of human annotation and machine propagation, both can have errors. Depth labels are output of a ML model (CREStereo) and hence can have errors as well. 
For the real sessions, the session level attributes are also human annotated and hence can also have errors.}

\item \question{Is the dataset self-contained, or does it link to or otherwise rely on external resources
(e.g., websites, tweets, other datasets)? If it links to or relies on external resources,
(a) Are there guarantees that they will exist, and remain constant, over time?
(b) Are there official archival versions of the complete dataset (i.e., including the external
resources as they existed at the time the dataset was created)?
(c) Are there any restrictions (e.g., licenses, fees) associated with any of the external resources
that might apply to a future user? Please provide descriptions of all external resources and
any restrictions associated with them, as well as links or other access points, as appropriate.}\\
\answer{SANPO dataset is self-contained and hosted by the Google Research Datasets team on Google Cloud storage. Short of organizational restructuring, we do not anticipate SANPO becoming unavailable for many years. (a) We might add newer versions in future. If we do so, then we will update the github readme accordingly. Older versions will remain usable but not recommended.
(b) Our institution hosts the only archive at the moment.
(c) Dataset is available under CC By 4.0 license. The accompanying code for its use is licensed under Apache 2.0.}

\item \question{Does the dataset contain data that might be considered confidential (e.g., data that is
protected by legal privilege or by doctor-patient confidentiality, data that includes the
content of individuals non-public communications)? If so, please provide a description.}\\
\answer{No.}

\item \question{Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety? If so, please describe why.}\\
\answer{No.}

\item \question{Does the dataset identify any subpopulations (e.g., by age, gender)? If so, please describe
how these subpopulations are identified and provide a description of their respective distributions
within the dataset.}\\
\answer{No.}

\item \question{Is it possible to identify one or more natural persons, either directly or indirectly (i.e., in combination with other data) from the dataset? If so, please describe how.}\\
\answer{It is possible. The videos were collected in public spaces, in accordance with local state and city laws. We have taken extra precautions to blur the PII, but some instances might not have been blurred.}

\item \question{Does the dataset contain data that might be considered sensitive in any way (e.g., data
that reveals racial or ethnic origins, sexual orientations, religious beliefs, political opinions
or union memberships, or locations; financial or health data; biometric or genetic data;
forms of government identification, such as social security numbers; criminal history)? If
so, please provide a description.}\\
\answer{This is highly unlikely as we blur the PII. But some instances of faces might not have been completely blurred.}

\item \question{Any other comments?}\\
\answer{No.}

\end{enumerate}

\section{Collection Process}
\begin{enumerate}

\item \question{How was the data associated with each instance acquired? Was the data directly observable
(e.g., raw text, movie ratings), reported by subjects (e.g., survey responses), or indirectly
inferred/derived from other data (e.g., part-of-speech tags, model-based guesses for age or
language)? If data was reported by subjects or indirectly inferred/derived from other data, was
the data validated/verified? If so, please describe how.}\\
\answer{The dataset was collected through an internal data collection effort. Some of the annotation are human annotated by contractors who work for Google's internal crowd labeling platform, and some annotations are machine generated.}

\item \question{What mechanisms or procedures were used to collect the data (e.g., hardware apparatus
or sensor, manual human curation, software program, software API)? How were these
mechanisms or procedures validated?}\\
\answer{We collected all data using hardware and compute resources provided by Google LLC. We built a hardware apparatus for volunteers to use. Post processing was done locally and then data upload to cloud. Details provided in the paper and in the appendix.}

\item \question{ If the dataset is a sample from a larger set, what was the sampling strategy?}\\
\answer{No.}

\item \question{Who was involved in data collection process (e.g., students, crowd-workers, contractors)
and how were they compensated (e.g., how much were crowd-workers paid)?}\\
\answer{The collection was done by Google's full time employees. Contracted human annotators were used for the human annotations. Parallel Domain provided the implementation and rendering of SANPO-Synthetic.}

\item \question{Over what timeframe was the data collected? Does this timeframe match the creation
timeframe of the data associated with the instances (e.g., recent crawl of old news articles)? If not, please provide a description of the timeframe.}\\
\answer{The dataset was collected in 2022 and 2023.}

\item \question{Were any ethical review processes conducted (e.g., by an institutional review board)? If
so, please provide a description of these review processes, including the outcomes, as well as a
link or other access point to any supporting documentation.}\\
\answer{Yes. The plan to collect data, safety of the volunteers, stability and ease of use of the hardware apparatus had to pass internal reviews as well as satisfy all the local state/city laws.}

\item \question{Does the dataset relate to people? If not, you may skip remaining questions in this section.}\\
\answer{No.}

\end{enumerate}

\section{Preprocessing, Cleaning, and/or Labeling}

\begin{enumerate}

\item \question{Was any preprocessing/cleaning/labeling of the data done (e.g., discretization or bucket-
ing, tokenization, part-of-speech tagging, SIFT feature extraction, removal of instances, processing of missing values)? If so, please provide a description. If not, you may skip the
remainder of the questions in this section.}\\
\answer{We used raw stereo videos to compute depth labels. All captured video went through a thorough PII removal (blurring of faces and license plates). Only PII removed data was saved and original raw data was deleted.}

\item \question{Was the “raw” data saved in addition to the preprocessed/cleaned/labeled data (e.g., to
support unanticipated future uses)? If so, please provide a link or other access point to the
“raw” data.}\\
\answer{No, we only provide the filtered data.}

\item \question{Is the software used to preprocess/clean/label the instances available? If so, please provide
a link or other access point.}\\
\answer{The model used to compute disparity based depth labels (CREStereo) is publicly available. The PII removal model is not publicly available, but we explain the process in detail in the paper, allowing
other researchers to reproduce our pipeline.}

\item \question{Any other comments?}\\
\answer{No.}

\end{enumerate}

\section{Uses}
\begin{enumerate}

\item \question{Has the dataset been used for any tasks already? If so, please provide a description.}\\
\answer{The dataset was used to trained models for Project Guideline. Details are in the application section of the main paper.}

\item \question{Is there a repository that links to any or all papers or systems that use the dataset? If so,
please provide a link or other access point.}\\
\answer{We do not maintain such a repository. However, citation trackers like Google Scholar and
Semantic Scholar would list all future works that cite our dataset.}

\item \question{What (other) tasks could the dataset be used for?}\\
\answer{The dataset could be used for any scene understanding related tasks.}

\item \question{Is there anything about the composition of the dataset or the way it was collected and
preprocessed/cleaned/labeled that might impact future uses? For example, is there anything
that a future user might need to know to avoid uses that could result in unfair treatment of
individuals or groups (e.g., stereotyping, quality of service issues) or other undesirable harms
(e.g., financial harms, legal risks) If so, please provide a description. Is there anything a future
user could do to mitigate these undesirable harms?}\\
\answer{If current or future users observe any PII which hasn't been properly blurred we request them to reach out to us with appropriate details via email to \texttt{sanpo\_dataset@google.com}. Other than that we don't anticipate in issues.}

\item \question{Are there any tasks for which the dataset should not be used? If so, please provide a
description.}\\
\answer{N/A.}

\item \question{Any other comments?}\\
\answer{No.}

\end{enumerate}


\section{Distribution}

\begin{enumerate}
    
\item \question{Will the dataset be distributed to third parties outside of the entity (e.g., company, insti-
tution, organization) on behalf of which the dataset was created? If so, please provide a description.}\\
\answer{Yes, our dataset is publicly available and does not require registration.}

\item \question{How will the dataset will be distributed (e.g., tarball on website, API, GitHub) Does the
dataset have a digital object identifier (DOI)?}\\
\answer{Our dataset is hosted on Google cloud. Our github repo provides instructions on how to download it. It doesn't have DOI.}

\item \question{When will the dataset be distributed?}\\
\answer{The dataset is public since October 9, 2023.}

\item \question{Will the dataset be distributed under a copyright or other intellectual property (IP) li-
cense, and/or under applicable terms of use (ToU)? If so, please describe this license and/or
ToU, and provide a link or other access point to, or otherwise reproduce, any relevant licensing
terms or ToU, as well as any fees associated with these restrictions.}\\
\answer{This data will be licensed by Google Inc. under a Creative Commons
Attribution 4.0 International License. Users will be allowed to modify and repost it, and we
encourage them to analyze and publish research based on the data.}

\item \question{Have any third parties imposed IP-based or other restrictions on the data associated
with the instances? If so, please describe these restrictions, and provide a link or other access
point to, or otherwise reproduce, any relevant licensing terms, as well as any fees associated
with these restrictions.}\\
\answer{No. Parallel Domain agreed to release SANPO-Synthetic on identical terms.}

\item \question{Do any export controls or other regulatory restrictions apply to the dataset or to individ-
ual instances? If so, please describe these restrictions, and provide a link or other access point
to, or otherwise reproduce, any supporting documentation.}\\
\answer{No.}

\item \question{Any other comments?}\\
\answer{No.}

\end{enumerate}

\section{Maintenance}
\begin{enumerate}
    
\item \question{Who will be supporting/hosting/maintaining the dataset?}\\
\answer{The authors will maintain the dataset. The dataset is hosted on Google cloud. All the information
about the dataset, including links to the paper and future announcements will be accessible at
the dataset website and github repo.}

\item \question{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?}\\
\answer{The contact emails of authors are available on the dataset website.}

\item \question{Is there an erratum? If so, please provide a link or other access point.}\\
\answer{There is no erratum for our initial release.}

\item \question{Will the dataset be updated (e.g., to correct labeling errors, add new instances, delete
instances)? If so, please describe how often, by whom, and how updates will be communicated
to users (e.g., mailing list, GitHub)?}\\
\answer{We will update our dataset periodically and announce updates on the dataset website.}

\item \question{If the dataset relates to people, are there applicable limits on the retention of the data
associated with the instances (e.g., were individuals in question told that their data would
be retained for a fixed period of time and then deleted)? If so, please describe these limits
and explain how they will be enforced.}\\
\answer{N/A.}

\item \question{Will older versions of the dataset continue to be supported/hosted/maintained? If so,
please describe how. If not, please describe how its obsolescence will be communicated to users.}\\
\answer{We will support older versions if there are no PII issues with them, otherwise they be removed and communicated via our github repo.}

\item \question{If others want to extend/augment/build on/contribute to the dataset, is there a mecha-
nism for them to do so? If so, please provide a description. Will these contributions be verified?
If so, please describe how. If not, why not? Is there a process for communicating/distributing
these contributions to other users? If so, please provide a description.}\\
\answer{Anyone can extend SANPO. We recommend reaching out to us via our email or by contacting \texttt{sanpo\_dataset@google.com}.}

\end{enumerate}

==> floats/data-capture.tex <==
\begin{figure}[th]%
    \centering
    \includegraphics[bb=0cm 0cm 15cm 11cm, width=.8\linewidth,clip]{figures/Data-Capture-Methodology_2.pdf}
    \caption{\textbf{Data capture methodology for SANPO.} SANPO contains a mix of both real and synthetic data. The real data is captured from a chest-mounted camera and a head-mounted camera, while the synthetic data comes from a virtual environment. Our videos have depth maps and panoptic segmentations.}%
    \label{fig:data-capture}%
\end{figure}

==> floats/sam.tex <==
\begin{figure}[t!]%
\centering
\includegraphics[bb=0 0 1400 1050, width=0.8\linewidth]{figures/images/sanpo_and_sam.png.jpg}%
\caption{\textbf{Segment Anything Model (SAM) on SANPO.}  We evaluated SAM on SANPO images. The middle column shows sample instance masks in SANPO and the selected point used to prompt SAM. The last column shows the predicted masks generated by SAM.}%
\label{fig:small_objects_mask}%
\end{figure}

==> floats/table-train-new.tex <==
\begin{table}
{

\centering

\begin{tabular}{ccccc}
\toprule

\multicolumn{5}{c}{\textbf{Panoptic Segmentation}}\\
\midrule

\textbf{Dataset} & \textbf{Method} & \textbf{Encoder} 
& \textbf{mIoU $\uparrow$}
& \textbf{PQ $\uparrow$}\\
\midrule

SANPO-Real-Train & Kmax-DeepLab \cite{yu2023kmaxdeeplab} & Resnet-50 \cite{he2016deep} & 43.4 & 34.6\\
SANPO-Real-Train & Kmax-DeepLab \cite{yu2023kmaxdeeplab} & ConvNeXt-L \cite{liu2022convnet} & 46.0 & \textbf{38.4}\\
\begin{tabular}{@{}c@{}}SANPO-Real-Train \\ (Human GT only)\end{tabular} & Kmax-DeepLab \cite{yu2023kmaxdeeplab} & Resnet-50 \cite{he2016deep} & 42.7 & 34.6\\
\begin{tabular}{@{}c@{}}SANPO-Real-Train \\ (Human GT only)\end{tabular} & Kmax-DeepLab \cite{yu2023kmaxdeeplab} & ConvNeXt-L \cite{liu2022convnet} & \textbf{46.5} & 38.2\\
\cmidrule(lr){1-5}
\begin{tabular}{@{}c@{}}SANPO-Real-Train \\ (Human GT only)\end{tabular} & DeepLabv3 \cite{chen2017rethinking} & MobilenetV3 \cite{howard2019searching} & 36.8 & \textdaggerdbl\\
\midrule

\multicolumn{5}{c}{Synthetic to Real Domain Adaptation}\\
\midrule

SANPO-Synthetic-Train	& Kmax-DeepLab \cite{yu2023kmaxdeeplab} & Resnet-50 \cite{he2016deep}	& 14.6	& 9.6\\
SANPO-Synthetic-Train	& Kmax-DeepLab \cite{yu2023kmaxdeeplab} & ConvNeXt-L \cite{liu2022convnet} & 17.6	& 11.1\\
\begin{tabular}{@{}c@{}}SANPO-Synthetic-Train ->\\ SANPO-Real-Train \\ (Human GT only)\text{*} \end{tabular}	& Kmax-DeepLab \cite{yu2023kmaxdeeplab} & Resnet-50 \cite{he2016deep} & 44.1 & 34.6\\
\begin{tabular}{@{}c@{}}SANPO-Synthetic-Train ->\\ SANPO-Real-Train \\ (Human GT only)\text{*} \end{tabular}	& Kmax-DeepLab \cite{yu2023kmaxdeeplab} & ConvNeXt-L \cite{liu2022convnet} & 47.0 & 38.3\\
\begin{tabular}{@{}c@{}}SANPO-Synthetic-Train +\\ SANPO-Real-Train \\ 80\% Synthetic \dag\end{tabular}	& Kmax-DeepLab \cite{yu2023kmaxdeeplab} & Resnet-50 \cite{he2016deep} & 40.7 & 31.2\\
\begin{tabular}{@{}c@{}}SANPO-Synthetic-Train +\\ SANPO-Real-Train \\ 80\% Synthetic \dag\end{tabular}	& Kmax-DeepLab \cite{yu2023kmaxdeeplab} & ConvNeXt-L \cite{liu2022convnet} & 45.2 & 35.4\\
\begin{tabular}{@{}c@{}}SANPO-Synthetic-Train +\\ SANPO-Real-Train \\ 50\% Synthetic \dag\end{tabular} & Kmax-DeepLab \cite{yu2023kmaxdeeplab} & Resnet-50 \cite{he2016deep} &	43.0 & 34.6\\
\begin{tabular}{@{}c@{}}SANPO-Synthetic-Train +\\ SANPO-Real-Train \\ 50\% Synthetic \dag \end{tabular} & Kmax-DeepLab \cite{yu2023kmaxdeeplab} & ConvNeXt-L \cite{liu2022convnet} & \textbf{48.1} & \textbf{38.3}\\

\midrule
\multicolumn{5}{c}{\textbf{Depth Estimation}}\\
\midrule
\textbf{Dataset} & \textbf{Method} & \textbf{Encoder}
%& &\\
& \multicolumn{2}{c}{\depthmetric{}$\uparrow$}\\
\midrule
SANPO-Real-Train	& BinsFormer \cite{li2022binsformer} & Resnet-50 \cite{he2016deep} & \multicolumn{2}{c}{0.45}\\
SANPO-Synthetic-Train	& BinsFormer \cite{li2022binsformer} & Resnet-50 \cite{he2016deep} & \multicolumn{2}{c}{0.27}\\

\bottomrule
\end{tabular}
}
\caption{\textbf{SANPO Benchmark.} \text{*}: Pretrained on synthetic and then fine-tuned on real. \dag : Trained on combined real and synthetic data. \textdaggerdbl: Mobile friendly quantized semantic segmentation model train on 512x512 resolution. 
%Segmentation models evaluated on SANPO-Real-Test (Human GT Only). Depth models evaluated on SANPO-Real-Test.
}
\label{table:train}
\end{table}

==> floats/table-train-synthetic-to-real.tex <==
\begin{table*}[t]
{
\centering

\begin{tabular}{ccccc}
\toprule

\textbf{Dataset} & \textbf{Method} & \textbf{Encoder} 
& \textbf{mIoU $\uparrow$}
& \textbf{PQ $\uparrow$}\\
\midrule

SANPO-Synthetic-Train	& Kmax-DeepLab \cite{yu2023kmaxdeeplab} & Resnet-50 \cite{he2016deep}	& 14.6	& 9.6\\
\begin{tabular}{@{}c@{}}SANPO-Synthetic-Train ->\\ SANPO-Real-Train$\ddagger$ \end{tabular}	& Kmax-DeepLab \cite{yu2023kmaxdeeplab} & Resnet-50 \cite{he2016deep} & 44.1 & 34.6\\
\begin{tabular}{@{}c@{}}SANPO-Synthetic-Train +\\ SANPO-Real-Train \\ 80\% Synthetic \dag\end{tabular}	& Kmax-DeepLab \cite{yu2023kmaxdeeplab} & Resnet-50 \cite{he2016deep} & 40.7 & 31.2\\
\begin{tabular}{@{}c@{}}SANPO-Synthetic-Train +\\ SANPO-Real-Train \\ 50\% Synthetic \dag\end{tabular} & Kmax-DeepLab \cite{yu2023kmaxdeeplab} & Resnet-50 \cite{he2016deep} &	43.0 & 34.6\\

SANPO-Synthetic-Train	& Kmax-DeepLab \cite{yu2023kmaxdeeplab} & ConvNeXt-L \cite{liu2022convnet} & 17.6	& 11.1\\
\begin{tabular}{@{}c@{}}SANPO-Synthetic-Train ->\\ SANPO-Real-Train $\ddagger$ \end{tabular}	& Kmax-DeepLab \cite{yu2023kmaxdeeplab} & ConvNeXt-L \cite{liu2022convnet} & 47.0 & 38.3\\
\begin{tabular}{@{}c@{}}SANPO-Synthetic-Train +\\ SANPO-Real-Train \\ 80\% Synthetic \dag\end{tabular}	& Kmax-DeepLab \cite{yu2023kmaxdeeplab} & ConvNeXt-L \cite{liu2022convnet} & 45.2 & 35.4\\
\begin{tabular}{@{}c@{}}SANPO-Synthetic-Train +\\ SANPO-Real-Train \\ 50\% Synthetic \dag \end{tabular} & Kmax-DeepLab \cite{yu2023kmaxdeeplab} & ConvNeXt-L \cite{liu2022convnet} & \textbf{48.1} & \textbf{38.3}\\

\bottomrule
\end{tabular}
\caption{\textbf{Synthetic Data Boosts Performance}. Incorporating synthetic data, either through pretraining or as a component of the training dataset, consistently improves performance. \text{->}: Pretrained on synthetic and then fine-tuned on real data. \text{+} : Trained on combined real and synthetic data. $\ddagger$: Human annotated GT only.}
\label{table:train-synthetic-to-real}

}
\end{table*}

==> sections/generic_rebuttal.tex <==
\section{Data Diversity Plots}
\begin{figure}[h]
\includegraphics[width=1.0\textwidth]{figures/images/label-distributions.pdf}
\caption{\textbf{Distribution of video-level attributes,} highlighting the diversity of scenes in SANPO.}
\end{figure}

\section{On-device Navigation specific Segmentation and Obstacle Detection}
\todo{Move to generic rebuttal markdown}

As mentioned in Sec.~6, SANPO serves as the flagship training set for \emph{Google Project Guideline}\cite{PROJECTGUIDELINE}, a mobile application platform that helps people who are blind or low-vision to walk or run for exercise independently. Project Guideline uses SANPO-trained mobile-friendly depth estimation and semantic segmentation models to help users navigate and avoid obstacles. (Though it is out of scope for our paper, interested readers can see the reference for the models' open source release.)

To evaluate model performance, we re-use SANPO's semantic segmentation and depth estimation annotations as a test bed for an outdoor obstacle detection and rangefinding task.
The goal is to measure how well SANPO-trained models can detect obstacle classes at various distances.

\textbf{Metrics.} For this task's labels, we mapped SANPO labels to ``safe for walking,'' ``not safe for walking,'' and ``obstacles''\footnote{Please refer to A.6.1 for the Accessibility taxonomy}. We select these abstract classes as they are crucial for navigation. Obstacles need both segmentation and distance estimation, while ground surfaces mainly require reliable segmentation. We report mIoU of this smaller taxonomy. For obstacle rangefinding, we report $\depthmetric~\uparrow$ of only obstacle classes, binning the metric at short range, medium range, and long range.

\textbf{Model training.} For semantic segmentation, we trained a quantized MobileNetV3 \cite{howard2019searching} with a input resolution of 512x512. For depth estimation, a small MidasNet model \cite{DBLP:journals/corr/abs-1907-01341} with a input resolution of 192x192.
Using these models, we establish a straightforward navigation specific benchmark.
Depth output is resized to 512x512, with metrics reported at this resolution (Table~\ref{table:accessibility-eval}).
\input{floats/accessibility_eval}


\section{SANPO-Synthetic Rendering Specifications}
Detailed specifications for SANPO-Synthetic's virtual rendering environment are available at \\ \url{https://gist.github.com/gcr/7850925067f552cfb0fb699fe6004b69}

\cut{
\section{Benchmarks and Accessibility}
\subsection{Zero-Shot Evaluation}
To do a rigorous zero-shot evaluation we evaluated SANPO on models trained on the Cityscapes and KITTI datasets as they are the most prominent datasets for semantic segmentation and depth estimation respectively. As requested by the reviewer we have also included the depth estimation performance on the Cityscapes-DVPS dataset \cite{vip_deeplab}.
\input{floats/table-zero-shot}
}
